Complementary Meta-Reinforcement Learning for Fault-Adaptive Control

Faults are endemic to all systems. Adaptive fault-tolerant control maintains degraded performance when faults occur as opposed to unsafe conditions or catastrophic events. In systems with abrupt faults and strict time constraints, it is imperative for control to adapt quickly to system changes to maintain system operations. We present a meta-reinforcement learning approach that quickly adapts its control policy to changing conditions. The approach builds upon model-agnostic meta learning (MAML). The controller maintains a complement of prior policies learned under system faults. This "library" is evaluated on a system after a new fault to initialize the new policy. This contrasts with MAML, where the controller derives intermediate policies anew, sampled from a distribution of similar systems, to initialize a new policy. Our approach improves sample efficiency of the reinforcement learning process. We evaluate our approach on an aircraft fuel transfer system under abrupt faults.

==> biographies.tex <==
\section*{Biographies}

\noindent\textbf{Ibrahim Ahmed} is a PhD student in Electrical Engineering at Vanderbilt University, Nashville, TN. He has a MS in Electrical Engineering (2018) and a BS in Electrical Engineering and Physics (2016) from the same university. His research focus is on fault-tolerant control using reinforcement learning. He is also interested in data-driven models of hybrid systems and energy optimization in smart buildings.

\noindent\textbf{Marcos Quiñones-Grueiro}

\noindent\textbf{Gautam Biswas}
